Quasi-matrix-free hybrid multigrid on dynamically adaptive Cartesian grids

We present a family of spacetree-based multigrid realizations using the tree's multiscale nature to derive coarse grids. They align with matrix-free geometric multigrid solvers as they never assemble the system matrices which is cumbersome for dynamically adaptive grids and full multigrid. The most sophisticated realizations use BoxMG to construct operator-dependent prolongation and restriction in combination with Galerkin/Petrov-Galerkin coarse-grid operators. This yields robust solvers for nontrivial elliptic problems. We embed the algebraic, problem- and grid-dependent multigrid operators as stencils into the grid and evaluate all matrix-vector products in-situ throughout the grid traversals. While such an approach is not literally matrix-free---the grid carries the matrix---we propose to switch to a hierarchical representation of all operators. Only differences of algebraic operators to their geometric counterparts are held. These hierarchical differences can be stored and exchanged with small memory footprint. Our realizations support arbitrary dynamically adaptive grids while they vertically integrate the multilevel operations through spacetree linearization. This yields good memory access characteristics, while standard colouring of mesh entities with domain decomposition allows us to use parallel manycore clusters. All realization ingredients are detailed such that they can be used by other codes.

==> 06bapp_distributed-memory.tex <==
\section{Remarks on the distributed memory parallelization}

Our top-down domain decomposition uses per level the Peano SFC to obtain
connected subpartitions with good
surface-to-volume ratio \cite{Bader:13:SFCs,Griebel:99:SFCAndMultigrid}.
Graph-based approaches would be another option.
They are notably promising candidates if the proposed
algorithms are extended to forests.

While the recursive top-down splitting proposed constrains the potential
fine-grid cuts and the strategy to deploy one cell per rank is naive, 
it automatically yields the master-worker topology.
Better splitting strategies are mandatory for real-world
experiments.
We notably refer to \cite{Schreiber:13:Cluster} or the opportunity to deploy
multiple MPI ranks per node to deploy multiple cells to one MPI rank. 

Furthermore, we emphasise that the knowledge about $\ell _{max}$ and $\ell _{min}$
allows an algorithm to skip most of the `wake-up calls' introduced in the
manuscript:
we know a priori how many tree sweeps we need for a cycle.
Each rank can trigger these sweeps which reduces the synchronisation points of
the ranks.
Only one additional, totally synchronised sweep is required in the end to
conduct grid refinement.
The level of asynchronism of such an approach is particularly high for $\mu > 1$ cycles
and not subject of study here.

The exchange of hierarchical stencil entries reduces the bandwidth requirements.
The send/receive semantics then is three-fold: 
If a local vertex's operators equal rediscretization or $d$-linear operators
respectively, we send out a simple flag.
On the receive side, this flag makes the receiving rank reconstruct the incoming
data through rediscretization.
If a local vertex's operator is not compressed we send out the whole operator.
Otherwise, we send out the $bpa$ bits and then the corresponding byte stream of
the operator.
The receiving side decompresses its local stencil, decompresses
the received data, and combines the two.


==> 08aapp_sin.tex <==
\section{Additional experimental data}

\begin{figure}[ht]
 \begin{center}
  %
  %  I had to rename the files as arXiv doesn't like me to have too long files
  %
  %  img20: convergence-speed-RegularPoisson-2d-0_8-GeometricBPX.pdf
  %  img21: convergence-speed-RegularPoisson-3d-0_8-GeometricBPX-no-legend.pdf
  %  img22: convergence-speed-RegularPoisson-2d-0_8-MultiplicativeGeometricV21-no-legend.pdf
  %  img23: convergence-speed-RegularPoisson-3d-0_8-MultiplicativeGeometricV21-no-legend.pdf
  %  img24: convergence-speed-RegularPoisson-2d-0_8-MultiplicativeGeometricV33-no-legend.pdf
  %  img25: convergence-speed-RegularPoisson-3d-0_8-MultiplicativeGeometricV33-no-legend.pdf
  %
  \includegraphics[width=0.35\textwidth]{experiments/convergence/sin/img20.pdf}
  \includegraphics[width=0.35\textwidth]{experiments/convergence/sin/img21.pdf}
  \includegraphics[width=0.35\textwidth]{experiments/convergence/sin/img22.pdf}
  \includegraphics[width=0.35\textwidth]{experiments/convergence/sin/img23.pdf}
%   \includegraphics[width=0.45\textwidth]{experiments/convergence/sin/img24.pdf}
%   \includegraphics[width=0.45\textwidth]{experiments/convergence/sin/img25.pdf}
 \end{center}
    \vspace{-0.4cm}
 \caption{
   Convergence of various solvers for 
   (2) on regular grids with $\omega = 0.8$.
   Solid lines with filled symbols use a Jacobi smoother, dashed
   lines use block Jacobi with one Gau\ss -Seidel sweep, and
   dotted lines for apply three sweeps.
   Empty symbols furthermore are for solving the coarse-grid problem exactly
   while solid symbols are for applying only $\mu _{pre}+\mu _{post} $ sweeps on
   the coarsest grid.
   \label{figure:experiments:sin:solvers}
 }
\end{figure}


\begin{table}[ht]
  \caption{
    Iteration counts for the additive multigrid, additive multigrid with exact
    coarse-grid solve, and BPX (left to right) with $\omega = 0.8$ solving
    \texttt{jump} for $d=2$.
    $\bot $ is used to denote that a solver was not able
    to reduce the residual by a factor of $10^{8}$ within 300 iterations.
    \label{results:jump:additive}
  }
{
\tiny
   \vspace{-0.3cm}
\begin{center}
 \setlength{\tabcolsep}{2.4pt}
 \begin{tabular}{l|ccccc|ccccc|ccccc}
   %
   % arXiv doesn't allow me to have long table names
   %
   % Original file:
   %
   % iterations-AdditiveGeometricMGWithExponentialDampingWithoutConsistentMultilevelRepresentation-Galerkin-2d-RegularJump.table
   %
   \input{experiments/convergence/jump/table00and10.table}
 \end{tabular}
\end{center}
}
\end{table}


The reported iteration counts in Section 6.1 can directly be taken from Fig.~\ref{figure:experiments:sin:solvers}.
Additional experiments for setup (3) with the additive multigrid solver and BPX
are given in Table \ref{results:jump:additive}.

